MV-IVF: Multi-Vector Retrieval via Multi-Vector Clustering

Multi-vector retrieval represents each query and document as a set of embeddings and scores relevance via fine-grained set-to-set interactions such as MaxSim (Chamfer similarity). This expressiveness improves retrieval quality over single-vector representations, but makes search substantially more expensive. Existing systems address this challenge primarily through proxy representations or filter-and-rerank pipelines that reduce candidate generation to single-vector search. We study the complementary direction of building a native IVF-style index directly over multi-vector data. We introduce MV-IVF, an inverted-file index for multi-vector retrieval built on MV-Lloyd, a new Lloyd-style algorithm for clustering point clouds under a Chamfer objective. Our key observation is that once point clouds are assigned to clusters, the center-update step reduces to standard single-vector clustering over the flattened embeddings in each cluster. This enables efficient construction of a hierarchical IVF tree with center point clouds at internal nodes. At query time, MV-IVF performs best-first beam search over the tree to identify promising leaf clusters, then scores the documents in those leaves. We further accelerate search using low-bit quantization, query compression, and cache-efficient batched search. We implement MV-IVF in MVSIC, an optimized C++ library and unified evaluation framework for multi-vector retrieval that includes several major approaches. Across BEIR and LoTTE text retrieval benchmarks, MV-IVF achieves strong latency--recall tradeoffs, the best batched throughput frontiers, and favorable build-time and index-size profiles. At $90\%$ Recall-$10$@$10$, MV-IVF achieves up to $8.03\times$ lower single-query latency and up to $173.5\times$ higher QPS than the baselines, demonstrating that native IVF-style indexing is practical and effective for scalable multi-vector retrieval.

==> algo/combined.tex <==
\begin{figure*}[t]
\centering

\begin{minipage}[t]{0.42\textwidth}
\IncMargin{1.2em}
\begin{algorithm}[H]
    \footnotesize
    \caption{\mvlloyd}\label{alg:mvlloyd}
    \Input{Collection of point clouds $\cP$, parameters $k,s,T$}
    \Output{Collection of $k$ point clouds $\cC = \{C_1,\ldots,C_k\}$, where $|C_i|=s$}
    \tcp{Initialization}
    Let $\cC \gets$ uniform random sample of $k$ point clouds from $\cP$\;

    \For{$t=1$ to $T$}{
        \tcp{Assign point clouds to nearest centers}
        \parfor{$i=1$ to $k$}{
            $\Pi(i) \gets \{P\in \cP: i=\argmin_{j\in [k]}\Chn(P,\cC(j))\}$\;
        }

        \tcp{Compute new centroid point clouds}
        \parfor{$i=1$ to $k$}{
            $\cC(i) \gets \textsc{kmeans}(\flatten(\Pi(i)),s)$\;
        }
    }
    \Return{$\cC$}
\end{algorithm}
\DecMargin{1.2em}
\end{minipage}
\hfill
\begin{minipage}[t]{0.55\textwidth}
\IncMargin{1.2em}
\begin{algorithm}[H]
    \footnotesize
    \caption{\textsc{GreedySearch}}
    \label{alg:greedy-search}
    \Input{Query point cloud $Q$, MVIVF tree $T$, \nprobe, and \beamsize}
    \Output{Top \nprobe leaf nodes to probe}

    Initialize a \emph{beam} with the root node of $T$\;
    Initialize an empty top-$k$ structure $\cL$ with $k = \nprobe$\;

    \While{the beam is non-empty}{
        Extract the best node $u$ from the beam\;

        \If{$|\cL|=\nprobe$ ~and~ $\maxsim(Q,u)\le \min_{v\in \cL} \maxsim(Q,v)$}{
            \textbf{break} \tcp*[r]{early termination}
        }

        Compute $\maxsim$ values from $Q$ to all children of $u$\;

        \ForEach{child $v$ of $u$}{
            \eIf{$v$ is a leaf}{
                insert $v$ into $\cL$ if it belongs to the current top \nprobe leaves\;
            }{
                insert $v$ into the beam if it belongs to the current top \beamsize internal nodes\;
            }
        }
    }
    \Return{$\cL$}
\end{algorithm}
\DecMargin{1.2em}
\end{minipage}
\vspace{-1.3em}
\end{figure*}


==> algo/combined_new.tex <==
\begin{figure*}[t]
\centering

\begin{algoinsidefig}{0.42\textwidth}
\IncMargin{1.2em}
\begin{algocf}
    % \footnotesize
\caption{\mvlloyd}\label{alg:mvlloyd}
    \Input{Collection of point clouds $\cP$, parameters $k,s,T$}
    \Output{Collection of $k$ point clouds $\cC = \{C_1,\ldots,C_k\}$, where $|C_i|=s$}

    \tcp{Initialization}
    Let $\cC \gets$ uniform random sample of $k$ point clouds from $\cP$\;

    \For{$t=1$ to $T$}{
        \tcp{Assign point clouds to nearest centers}
        \parfor{$i=1$ to $k$}{
            $\Pi(i) \gets \{P\in \cP: i=\argmin_{j\in [k]}\Chn(P,\cC(j))\}$\;
        }

        \tcp{Compute new centroid point clouds}
        \parfor{$i=1$ to $k$}{
            $\cC(i) \gets \textsc{kmeans}(\flatten(\Pi(i)),s)$\;
        }
    }
    \Return{$\cC$}
\end{algocf}
\DecMargin{1.2em}
\end{algoinsidefig}
\hfill
\begin{algoinsidefig}{0.55\textwidth}
\IncMargin{1.2em}
\begin{algocf}
    \footnotesize
    \caption{\textsc{GreedySearch}}\label{alg:greedy-search}
    \Input{Query point cloud $Q$, MVIVF tree $T$, \nprobe, and \beamsize}
    \Output{Top \nprobe leaf nodes to probe}

    Initialize a \emph{beam} with the root node of $T$\;
    Initialize an empty top-$k$ structure $\cL$ with $k = \nprobe$\;

    \While{the beam is non-empty}{
        Extract the best node $u$ from the beam\;

        \If{$|\cL|=\nprobe$ ~and~ $\maxsim(Q,u)\le \min_{v\in \cL} \maxsim(Q,v)$}{
            \textbf{break} \tcp*[r]{early termination}
        }

        Compute $\maxsim$ values from $Q$ to all children of $u$\;

        \ForEach{child $v$ of $u$}{
            \eIf{$v$ is a leaf}{
                insert $v$ into $\cL$ if it belongs to the current top \nprobe leaves\;
            }{
                insert $v$ into the beam if it belongs to the current top \beamsize internal nodes\;
            }
        }
    }
    \Return{$\cL$}
\end{algocf}
\DecMargin{1.2em}
\end{algoinsidefig}

\vspace{-1.3em}
\end{figure*}

==> tables/datasets.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{ccccc}
\toprule
  Dataset &
  Corpus Size &
  Num Queries &
  Avg \# Embs per Doc  &
  License \\
\midrule
  {\tt nfcorpus}      & 3.6K & 323 & 235.49 & CC BY-SA 4.0\\
     {\tt scifact}    & 5.1K & 300 & 235.65 &  CC BY-NC 2.0\\
     {\tt arguana}    & 8.6K & 1,406 & 154.72 & Apache-2.0\\
     {\tt scidocs}    & 25.6K & 1,000 & 165.05 & CC BY 4.0\\
     {\tt fiqa}       & 57.6K & 648 & 126.9 & CC BY-SA 4.0\\
     {\tt nq}         & 2.68M & 3,452 & 100.3 & Apache-2.0\\
     {\tt hotpotqa}   & 5.23M & 7,405 & 68.65 & CC BY-SA 4.0 \\
     {\tt msmarco}    & 8.84M & 6,980 & 78.8 & CC BY-SA 4.0 \\
     {\tt lotte (pooled)}   & 2.4M    & 2,931 & 141.2  & Apache-2.0\\
% \midrule 
% % \multirow{5}{*}{\begin{sideways}LoTTE\end{sideways}} 
% %      & {\tt Writing}     &  &  &  & \\
% %      & {\tt Recreation}  &  &  &  & \\
% %      & {\tt Science}     &  &  &  & \\
% %      & {\tt Technology}  &  &  &  & \\
% %      & {\tt Lifestyle}   &  &  &  & \\
% % \midrule 
% \multirow{5}{*}{\begin{sideways}ViDoRe\end{sideways}} 
%      & {\tt DocVQA}    & 500 & 451 & 1030 & \\
%      & {\tt InfoVQA}   & 500 & 494 & 1030 & \\
%      & {\tt TAT-DQA}   & 271 & 1646 & 1030 & \\
%      & {\tt arXiVQA}   & 500 & 500 & 1030 & \\
%      & {\tt TabFQuAD}  & 70 & 280 & 1030 & \\
\bottomrule
\end{tabular}
\caption{\small Datasets used in this paper.}
\label{tab:datasets}
\end{table*}

==> tables/recall100_speedups.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llccc}
\toprule
Regime & Baseline & 90\% Recall-$100$@$100$ & 95\% Recall-$100$@$100$ & 99\% Recall-$100$@$100$ \\
\midrule
\multirow{3}{*}{Latency}
  & MUVERA    & $2.46\times$ / $4.50\times$ (6) & $3.14\times$ / $3.96\times$ (5) & $2.63\times$ / $4.13\times$ (4)$^\dagger$ \\
  & SVH       & $3.08\times$ / $4.06\times$ (5) & $3.79\times$ / $5.06\times$ (5) & $2.91\times$ / $3.99\times$ (4)$^\dagger$ \\
  & MV-Vamana & $2.20\times$ / $3.68\times$ (6) & $2.49\times$ / $3.12\times$ (5) & $2.09\times$ / $2.62\times$ (4)$^\dagger$ \\
\midrule
\multirow{3}{*}{Throughput}
  & MUVERA    & $6.06\times$ / $26.55\times$ (8) & $6.03\times$ / $16.00\times$ (5) & $3.68\times$ / $5.93\times$ (4)$^\dagger$ \\
  & SVH       & $6.66\times$ / $32.24\times$ (8) & $4.63\times$ / $12.16\times$ (6) & $18.78\times$ / $80.08\times$ (5) \\
  & MV-Vamana & $2.69\times$ / $5.34\times$ (9) & $3.14\times$ / $4.86\times$ (9) & $2.77\times$ / $4.03\times$ (5) \\
\bottomrule
\end{tabular}
\caption{\small \textbf{MVIVF speedups at fixed Recall-$100$@$100$.} Each cell reports average speedup / maximum speedup over the baseline, with the number of datasets compared in parentheses. Latency speedup is baseline latency divided by \mvivf latency; throughput speedup is \mvivf QPS divided by baseline QPS. $^\dagger$ marks cells covering fewer than half of the nine evaluated datasets.}
\label{tab:recall100-speedups}
\end{table*}


==> tables/recall10_speedups.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llccc}
\toprule
Regime & Baseline & 90\% Recall-$10$@$10$ & 95\% Recall-$10$@$10$ & 99\% Recall-$10$@$10$ \\
\midrule
\multirow{3}{*}{Latency}
  & MUVERA    & $1.85\times$ / $4.76\times$ (9) & $2.24\times$ / $4.51\times$ (6) & $2.16\times$ / $2.92\times$ (3)$^\dagger$ \\
  & SVH       & $3.03\times$ / $8.03\times$ (8) & $4.21\times$ / $8.86\times$ (6) & $17.03\times$ / $31.09\times$ (4)$^\dagger$ \\
  & MV-Vamana & $1.76\times$ / $5.13\times$ (9) & $2.12\times$ / $3.35\times$ (6) & $3.45\times$ / $4.98\times$ (4)$^\dagger$ \\
\midrule
\multirow{3}{*}{Throughput}
  & MUVERA    & $3.08\times$ / $8.40\times$ (9) & $2.66\times$ / $6.97\times$ (7) & $2.91\times$ / $6.28\times$ (3)$^\dagger$ \\
  & SVH       & $25.94\times$ / $173.53\times$ (8) & $12.31\times$ / $42.85\times$ (7) & $515.48\times$ / $1482.60\times$ (4)$^\dagger$ \\
  & MV-Vamana & $2.46\times$ / $4.99\times$ (9) & $2.55\times$ / $4.77\times$ (8) & $6.20\times$ / $11.65\times$ (4)$^\dagger$ \\
\bottomrule
\end{tabular}
\caption{\small \textbf{MVIVF speedups at fixed Recall-$10$@$10$.} Each cell reports average speedup / maximum speedup over the baseline, with the number of datasets compared in parentheses. Latency speedup is baseline latency divided by \mvivf latency; throughput speedup is \mvivf QPS divided by baseline QPS. $^\dagger$ marks cells covering fewer than half of the nine evaluated datasets.}
\label{tab:recall10-speedups}
\end{table*}

